Hybrid Optimization Methods for Parameter Estimation of Reactive Transport Systems

This paper presents a hybrid optimization methodology for parameter estimation of reactive transport systems. Using reduced-order advection-diffusion-reaction (ADR) models, the computational requirements of global optimization with dynamic PDE constraints are addressed by combining metaheuristics with gradient-based optimizers. A case study in preparative liquid chromatography shows that the method achieves superior computational efficiency compared to traditional multi-start methods, demonstrating the potential of hybrid strategies to advance parameter estimation in large-scale, dynamic chemical engineering applications.

==> tex/old/chromatography.tex <==
\section{Chromatography case study}\label{sec:casestudy}

Chromatography unfolds in a column packed with porous particles forming the stationary phase. A component mixture, suspended in a liquid buffer (the mobile phase), courses through the column. Components adsorb to the stationary phase with varying affinities, resulting in distinct retention times forming the basis for separation. An eluent salt component, is often introduced to the system which disrupts interactions between the mobile and stationary phases. By controlling the trajectory of the eluent, the separation is further enhanced.

%We follow the case study presented in \cite{chen2024standardized}, which considers the separation of proteins using ion-exchange chromatography. Immunoglobulin G (IgG) antibodies are separated from a mixture of IgG, bovine serum albumin (BSA), and myoglobin (Mb). Sodium chloride (NaCl) is introduced as an MPM and its trajectory is optimized for a variety of objectives. To this end, we first describe the model introduced in \cite{Karlsson:2004}.

We follow a case study presented in \cite{chen2024standardized}, which considers the separation of industrial antibody feed mixture using ion-exchange chromatography. The case-study outlines and follows a detailed approach for accurate model development. Preliminary pulse-injection and titration experiments are conducted to estimate and validate the system and column specific parameters. Subsequently, bind-and-elution experiments are conducted where outlet absorbance and conductivity measurements are collected for model calibration. %The antibody feed mixture is split into 3 species for modeling purposes, A1 and A2 represent 2 impurity species and M is the desired product. To this end, we first describe the model introduced in \cite{chen2024standardized}.

The antibody feed mixture is considered to consist of three species, A1 and A2 representing two impurity species, and M the desired product. In this case study, we use the information collected by \cite{chen2024standardized} and implement our methods for model calibration, estimating isotherm parameters that describe how each component interacts with the stationary phase under varying loadings and eluent trajectories. With the calibrated model, we then subsequently perform process optimization to enhance separation efficiency and product yield.

To proceed, we first describe the chromatography model introduced in \cite{chen2024standardized}.

\subsection{Chromatography model}
Mathematical models of chromatography are two-fold: a column model capturing transport through the interstitial volume, and a kinetic model describing adsorption to and desorption from the stationary phase. The literature on mathematical models for chromatography is extensive and is perhaps best summarized by \cite{Guiochon:2006}. In practice, one-dimensional reduced-order models considering only advection and diffusion are commonplace. 

We study a column model known as the equilibrium dispersive model. A column of length $L$, volume $V$, and porosity $\varepsilon$ is modeled axially by $\Omega = [0,L]$. The transport of protein mobile phase concentrations is governed by Darcy's law and is described by the ADR system \eqref{eq:ADR} with boundary conditions \eqref{eq:BCs}, reactive components $\mathcal{C} = \mathcal{C}_q = \{\text{A1}, \text{A2}, \text{M}\}$, interstitial velocity $v = v_\text{in}$, and apparent diffusion coefficient $D = D_\text{app}$. The reaction term $R$ describes the adsorption of proteins on the stationary phase. We let $q$ denote the vector of stationary phase concentrations of bound proteins, and write
\begin{align}
    R(c) = - \phi \partial_t q,
\end{align}
where $\phi = (1-\varepsilon)/\varepsilon$ denotes the liquid volume fraction. Note that stationary phase concentrations may fit within the present framework of \eqref{eq:ADR} by appending stationary components. We use \eqref{Rstochiometry} with components $\mathcal{C}$ described by
\begin{align}
    c = [c_\text{salt}, c_\text{A1}, c_\text{A2}, c_\text{M}, q_\text{salt},q_\text{A1}, q_\text{A2}, q_\text{M}],
\end{align}
reaction rates $r= \partial_t q$, and stoichiometric matrix
\begin{align}
    \nu = \left[\begin{array}{ccc}
    -\phi I; & I
    \end{array}\right].
\end{align}


Table \ref{tb:Column} summarizes the column model parameters.

\begin{table}[tb]
\begin{center}
\caption{Column parameters}\label{tb:Column}
\begin{tabular}{cccccc}
$L$ {[}mm{]}         & $V$ {[}mm$^3${]}     & $\varepsilon_t$ {[}---{]} & $v$ {[}mm/s{]} & $D$ {[}mm$^2$/s{]} & $\Lambda$ {[}mol/l{]} \\ \hline
$192$ & $1.5072\cdot 10^{4}$ & 0.831                    & $0.7702$       & $9.56\cdot 10^{-2}$  & $0.64$           
\end{tabular}
\end{center}
\end{table}

The kinetic model is given by a multi-component steric mass action  isotherm. Given $i \in \mathcal{C}_q$, we write
\begin{subequations}\label{eq:Langmuir}
\begin{align}
    k_{\text{kin},i} \partial_t q_i = & k_{\text{eq},i}\left( \Lambda - \sum_{j \in \mathcal{C}_q}\left(\nu_j +\sigma_j\right) q_i \right)^{\nu_i} c_i - q_i c_\text{salt}^{\nu_i}\\
    &\partial_tq_{\text{salt}} = - \sum_{j \in \mathcal{C}_q}\nu_j \partial_tq_j
\end{align}
\end{subequations}

%where $q_{\text{max},i}$ denotes its maximum stationary phase concentration, $k_{\text{ads},i}$ denotes its adsorption rate, and $k_{\text{des},i}$ denotes its desorption rate. The rates are parameterized in \cite{Karlsson:2004} to incorporate information about the MPM. The resulting rates are given by
%\begin{subequations}\label{eq:MPM}
% \begin{align}
%     k_{\text{ads},i} &= k_{\text{ads}0,i} \exp({\gamma_i c_\text{NaCl}}),\\
%     k_{\text{des},i} &= k_{\text{des}0,i} c_\text{NaCl}^{\beta_i}.\label{eq:MPMdes}
% \end{align}
% \end{subequations}
Here $k_{\text{kin},i}$ denotes the kinetic coefficient, $ k_{\text{eq},i}$ denotes the equilibrium coefficient, $\Lambda$ describes the ionic capacity of the column, $\nu_i$ is a parameter which describes the protein characteristic charge, $\sigma_i$ describes the protein shielding factor.% The eluent component is assumed to be inert, i.e. $\partial_t q_\text{NaCl} = 0$.
% \begin{table}[tb]
% \begin{center}
% \caption{Isotherm parameters}\label{tb:Isotherm}
% \begin{tabular}{@{\hskip -0.025em}l@{\hskip -0.025em}cccc@{\hskip -0.025em}}
%                                      & Unit  & IgG     & BSA     & Mb      \\ \hline
% $q_{\text{max}, i}$ & [kmol/m$^3$]      & $5.40\cdot10^{-4}$ & $1.04\cdot10^{-3}$ & $7.50\cdot10^{-4}$ \\
% $k_{\text{des},i}$ &[kmol/(m$^3$min)] & $3.00\cdot10^{3}$ & $3.00\cdot10^{3}$ & $3.00\cdot10^{3}$ \\
% $k_{\text{ads},i}$ &[kmol/(m$^3$min)] & $2.31\cdot10^{6}$ & $1.76\cdot10^{5}$ & $5.00\cdot10^{6}$ \\
% $\gamma_i$ &[m$^3$/kmol] & 0.00 & 0.00 & 0.00\\
% $\beta_i$ &[---]                        & 1.12    & 3.20     & 0.61   
% \end{tabular}
% \end{center}
% \end{table}


\subsection{Process description}
The bind-and-elute experiments are performed as a batch process and can be divided into 3 sequential phases after the column has been initially equilibrated with low salt concentration buffer A (listed below)
\begin{enumerate}
    \item Loading phase: The feed mixture is injected into the column. 
    \item Washing phase: Weakly bound impurities are washed out using the low-salt buffer.
    \item Elution Phase: The salt concentration is increased and feed components eluted from the column.
\end{enumerate}

Two salt buffers are mixed together to control the salt concentration in the column

\begin{enumerate}
    \item Buffer A (low-salt buffer): 50 mM acetate.
    \item Buffer B (high-salt buffer): 50 mM acetate with 500 mM NaCl
\end{enumerate}

In the case study following \cite{chen2024standardized}, data from six different experiments were collected to calibrate and validate the chromatography model. Five gradient-elution experiments serve as the training set, and one step-elution experiment is used as a test set for model validation.

The same feed mixture is considered for all 6 experiments, it is considered as a mixture of 3 components. Two impurities labeled A1 and A2, and the desired product M. The concentration of each component in the mixture is analysed and listed in Table \ref{tb:Inlets}.

\begin{table}[tb]
\begin{center}
\caption{Feed concentrations}\label{tb:Inlets}
\begin{tabular}{ccccc}
           &Unit &  A1      & A2    & M    \\ \hline
 $c_\text{in,i}$ &[mol/l] &$2.895\cdot 10^{-5}$     & $1.558\cdot 10^{-5}$       & $6.750\cdot 10^{-5}$ 
\end{tabular}
\end{center}
\end{table}

In all gradient-elution experiments, the salt concentration is increased linearly from 0\% to 50\% Buffer B during the elution phase. While in the validation step-elution experiment the salt concentration is increased with a step from  0\% to 25\% Buffer B during the elution. The details of the variation among the experiments is listed in Table \ref{tb:ProcessDescription}. 

\begin{table}
\begin{center}
\caption{Process phases of all experiments}\label{tb:ProcessDescription}
\begin{tabular}{cccccc}
\hline
\multicolumn{1}{c}{Exp} & \multicolumn{1}{c}{Loading} & \multicolumn{1}{c}{{Washing}} & \multicolumn{1}{c}{{Elution}} & {Type} & {Purpose} \\
no. & {[CV]} & {[CV]} & {[CV]} & & \\
\hline
1 & 0.52 & 2 & 10 & Gradient & Calibration \\
2 & 0.52 & 2 & 15 & Gradient & Calibration \\
3 & 0.52 & 2 & 20 & Gradient & Calibration \\
4 & 1.56 & 2 & 10 & Gradient & Calibration \\
5 & 2.08 & 2 & 10 & Gradient & Calibration \\
6 & 0.52 & 2 & 5 & Step & Validation \\
\hline
\end{tabular}
\end{center}
\end{table}

% \begin{table}[tb]
% \begin{center}
% \caption{Process phases}\label{tb:Phases}
% \begin{tabular}{cccccc}
%   & Unit    & Load    & Elution  & Strip \\ \hline
% Duration &[min]        & 8             & Variable & 6     \\
% $c_\text{in,NaCl}$ & [kmol/m$^3$] & $9.00\cdot 10^{-3}$ & Variable & 1.00 
% \end{tabular}
% \end{center}
% \end{table}

\subsection{Chromatographic optimization}
Separation quality is quantified by an objective function, of which there are several in chromatographic optimization. 
Process yield and purity become increasingly important when the target protein is very expensive. The yield of IgG is defined at the column outlet as
\begin{align}\label{eq:Yield}
    Y = \frac{\int_{t_1}^{t_2}c_{\text{IgG}} \,\mathrm{d}t}{t_{\text{load}}c_{\text{in},\text{IgG}}},
\end{align}
where $c_{\text{in},\text{IgG}}$ is given in Table \ref{tb:Inlets}, $t_{\text{load}}$ is the duration of the loading phase, and $t_1,t_2$ are cut times for fraction collection. The fraction collection duration is constrained by a given purity requirement. Outlet purity is defined as
\begin{align}
    \Pi = \frac{c_\text{IgG}}{\sum_{j \in \mathcal{C}_q} c_j},
\end{align}
and we seek $\Pi \geq 99\%$. However, the cost of materials (stationary phase) and the cost of time may also dominate the execution of the process. Under these circumstances, a productivity objective is more important. We define productivity considering only the cost of time
\begin{align}\label{eq:Productivity}
    P = \frac{Y}{t_\text{tot}},
\end{align}
where $t_\text{tot}$ is the total process duration. To keep our exposition short, we fix the loading and stripping times, keeping the elution time variable, and consider only open-loop optimal controls maximizing the IgG yield. Table \ref{tb:Phases} summarizes the process phases.

\begin{figure}[tb]
\begin{center}
\adjustbox{trim=0 0.55cm 0 0cm}{\includegraphics[width=8.4cm]{figures/suboptimal_operation.pdf}}    % The printed column width is 8.4 cm.
\caption{Outlet profiles for optimal gradient elution with duration $T=40$ min.} 
\label{fig:subopt}
\end{center}
\end{figure}

The majority of literature on chromatographic optimization has shown linear (gradient) and single-step trajectories to be effective for separation. However, the constraint on the trajectory shape has the disadvantage of providing suboptimal solutions compared to multi-step or convex-concave trajectories (see \cite{Holmqvist:2016} and the references therein). Figure \ref{fig:subopt} shows an optimal gradient trajectory for the given process with fraction collection shaded in blue.

\begin{figure}[tb]
\begin{center}
\adjustbox{trim=0 0.55cm 0 0.0cm}{\includegraphics[width=8.4cm]{figures/optimal_controls.pdf}}  % The printed column width is 8.4 cm.
\caption{Outlet profiles for optimal controls for $N_\mathcal{S} = 8$ (solid) and $N_\mathcal{S} = 24$ (dashed) shooting intervals.} 
\label{fig:optcont}
\end{center}
\end{figure}
\begin{figure}[tb]
\begin{center}
\adjustbox{trim=0 0.55cm 0 0cm}{\includegraphics[width=8.4cm]{figures/optimal_operation.pdf}}  % The printed column width is 8.4 cm.
\caption{Outlet profiles for optimal controls with duration $T=32$ min (top) and $T=40$ (bottom).} 
\label{fig:goodyield}
\end{center}
\end{figure}

\subsection{Numerical experiments}


For most chromatography systems the individual component concentrations cannot be directly measured by optical sensors. Instead the UV-absorbance is measured at the column outlet. The observed UV-absorbance can be modeled as the linear combination of the simulated individual component concentrations using the Beer-Lambert law. At discrete time point $t_k$ the UV-absorbance at the outlet can be estimated for some model parameters $p$ as 
\begin{equation}
    y^{\text{UV}}(t_k, p) = \sum_{i=1}^{N_c} a_i c_{h,i}(t_k, p)|_{z = L}
\end{equation}
with the scaling factor $a_i = M_{w,i} \lambda_i l$, where $M_{w,i}$, $\lambda_i$ are the molecular weight and extinction coefficients of component $i$ respectively, $l$ the path length of the UV-sensor. $N_c$ is the number of components.

To further aid the calibration process, fractionation measurements are utilized. Fractionation involves collecting the effluent from the chromatography column into a series of sequential vials over time. Each vial, corresponding to a specific time interval, is then analyzed offline to quantify the components of interest. The fractionation data is often sparse, only containing 5-10 fractions per peak.

We model the fraction measurements as the average simulated outlet concentrations of component $i$ over a specified time interval $t_f = [t_f^{\text{start}},t_f^{\text{end}}]$%, $f \in [1,2,..., N_{\text{FRAC}}]$ as
\begin{equation}
    y^{\text{FRAC}}_i(t_f, p) = \frac{1}{t_f^{\text{end}} - t_f^{\text{start}}} \int_{t_f^{\text{start}}}^{t_f^{\text{end}}} c_{h,i}(t, p)|_{z=L} dt
\end{equation}



A trust-region reflective method is employed to solve the non-linear least squares problem defined in \eqref{eq:least_squares_objective}, using the solutions found by NSGA2 as initial values. To solve the least-squares problem we use accurate self-computed gradient information by constructing the residual Jacobian of the least squares objective function. The residual Jacobian is constructed from the gradients of UV and fractionation residuals defined in \eqref{eq:uv_residuals} and \eqref{eq:frac_residuals}.   

The gradient of the UV residual with respect to the $j$'th parameter $p_j$ is derived as
\begin{equation}
    \frac{\partial r^{\text{UV}}_n(t_k, p)}{\partial p_j} = w_n^{\text{UV}} \sum_{i=1}^{N_c} a_i \frac{\partial c_{h,i}^n(t_k, p)|_{z = L}}{\partial p_j}
\end{equation}

Whereas the gradient of the fractionation residual with respect to $p_j$ is derived as

\begin{equation}
    \frac{\partial r^{\text{FRAC}}_{n,i}(t_k, p)}{\partial p_j} = w_{n,i}^{\text{FRAC}} \frac{1}{t_f^{\text{end}}-t_f^{\text{strart}}} \int_{t_f^{\text{start}}}^{t_f^{\text{end}}} \frac{\partial c_{h,i}^n(t_k, p)|_{z = L}}{\partial p_j} dt
\end{equation}


The sensitivities of the estimated outlet concentrations $\partial c_{h,i}^n(t_k, p)|_{z = L} / \partial p_j$ are found using the forward sensitivity analysis approach described in Section \ref{sec:forward_sensitivities}.

\subsection{Local optimization}
The most efficient local optimization methods are gradient-based, which rely on accurate gradient information for good performance. In dynamic optimization problems, gradients are typically computed via sensitivity analysis, using either forward or adjoint methods depending on the problem size and structure. Incorporating second-order information, such as the Hessian, can further enhance convergence, offering local quadratic convergence. For least-squares problems, the Hessian is often approximated by the Gauss-Newton method, which neglects second-order residual terms. This approximation is computationally efficient and works well within Levenberg-Marquardt schemes, providing robust performance even for nonlinear problems.

% @ rel_tol = abs_tol = 1e-10
%                  order, n_el
% Step monotone,       3, 10 = 40 DOFS
% Step acceptable,     4, 5 = 25 DOFS
% Gradient monotone,   3, 5 = 20 DOFS 
% Gradient acceptable, 2, 5 = 15 DOFS
% Nominal integration scales linearly, but sensitivity calculations (using forward sensitivity analysis) will scale atleast quadratically due to sensitivity system solves

% @ rel_tol = 1e-3, abs_tol = 1e-7 works fine both for nominal integration and gradient-based
% approximate_sens a la Kristensen also works fine, but better for TRBDF2 than KENCARP47
% TRBDF2 is slightly slower for nominal integration, but faster for sensitivity generation


We will improve upon the gradient elution trajectory using the numerical methods described in the previous sections. We discretize the column with DG-FEM, choosing third-order polynomials $p=3$, and $N_\mathcal{E} = 10$ elements as a good compromise between solution accuracy and problem dimension. ESDIRK is used for the numerical integration and sensitivity generation, and we choose a relative tolerance of $10^{-6}$ and an absolute tolerance of $10^{-8}$ to account for the problem scaling. Stricter tolerances are used to simulate the concentration profiles after optimization. We solve the OCP with multiple shooting, and the number of shooting intervals is chosen as $N_\mathcal{S} \in \{8, 24\}$, which results in NLP problems with 2528 and 7024 decision variables, respectively. We optimize with respect to yield \eqref{eq:Yield}, and report the resulting productivity with respect to elution durations $T \in \{32, 40\}$ min. To account for fraction collection, we implement smoothed exact cut times. We consider a sigmoid
\begin{align}
    \sigma(x) = 1/(1+\exp(-(x/\delta)),
\end{align}
with shape parameter $\delta>0$, and we define the objective function from \eqref{eq:OCP} with spatial term $\psi_1 = 0$ and outlet term
\begin{align}
    \psi_2 = -\frac{\sigma(\Pi - 0.99)c_\text{IgG}}{t_{\text{load}}c_{\text{in},\text{IgG}}},
\end{align}
such that we minimize the negative yield during fraction collection. We choose $\delta = 0.01$, and report the exact yield and productivity of the resulting optimal controls.

As is usual for NLP problems, it is important to consider problem scaling and the choice of good initial guesses. We solve the resulting NLP with IPOPT \citep{Wachter:2006}, which is equipped with automatic scaling options. To make the solver more robust, we include box-constraints that prevent states and controls from taking significant unphysical values which could make the integration fail. Our strategy for choosing good initial guesses is described as follows. The optimal gradient control is found and interpolated onto $N_\mathcal{S}$ shooting intervals. Using the initial loaded state, the elution trajectory is integrated with strict tolerances yielding initial shooting states. Since the problem suffers from suboptimal local minima, the interpolated control is randomly perturbed to obtain an ensemble of initial control guesses. We optimize these, seeking controls that satisfy a convergence tolerance of $\text{tol} = 10^{-8}$, and we choose the optimal control with the maximum yield. This procedure is then repeated for finer multiple shooting discretizations by interpolation of the newly found optimal control. The individual solution times can vary significantly, ranging in the order of several minutes, and we found that considering ensembles with hundreds of initial guesses was necessary.

The optimal multi-step trajectories are shown in Figure \ref{fig:optcont}. Compared to the optimal gradient trajectory for $T=40$ min, the IgG peaks are significantly higher and better separated from the Mb and BSA peaks. This can also be seen in the consequent yield and purity results shown in Figure \ref{fig:goodyield} for $N_\mathcal{S} = 24$, improving upon the optimal gradient trajectory. For $T=32$ min the optimal gradient trajectory degrades performance, recovering less than $86\%$ in the elution phase. In comparison, the optimal multi-step trajectory has near unchanged performance, showing a $-1.1\%$ yield loss and a $0.39${$\,\%/$min} productivity gain. This demonstrates the competitive nature of the yield and productivity objectives.





\section{New model}
Accordingly, we consider the equilibrium dispersive column model, which is fits within the framework of the ADR systems presented in Section \ref{sec:modeling}. The column is
characterized by its length $L$, and is modeled axially as $\Omega = [0, L]$. The transport of the liquid buffer is described by the ADR system \eqref{eq:ADR} with inflow-outflow boundary conditions \eqref{eq:BCs} and diffusion motivated by Darcy's law of fluid flow in porous media. The system includes four components
\begin{align}
    \mathcal{C}_q = \{\text{NaCl}, \text{A1}, \text{A2}, \text{M}\},
\end{align}
each with their own mobile and stationary phase. Consequently, the component mixture $\mathcal{C}$ is described by a vector of mobile phases $c_i$ and stationary phases $q_i$ concentrations
\begin{align}
    c = [c_\text{salt}, c_\text{A1}, c_\text{A2}, c_\text{M}, q_\text{salt},q_\text{A1}, q_\text{A2}, q_\text{M}].
\end{align}
The velocities of the mobile components are defined by the interstitial velocity $v\text{in}$ and their diffusion coefficients by the apparent diffusion coefficient $D_\text{app}$. The adsorption between the mobile and stationary phases is described by the reaction term, which can be compactly expressed using~\eqref{Rstochiometry}. The stoichiometric matrix is defined as
\begin{align}
    \nu = \left[\begin{array}{cc}
    -\phi I; & I
    \end{array}\right],
\end{align}
where $\phi = (1-\varepsilon)/\varepsilon$ denotes the liquid volume fraction characterized by the column porosity $\varepsilon$. The associated kinetic rates $r = \partial_t q$ are given by a multi-component steric mass action isotherm. Given $i \in \mathcal{C}_q$, we write
\begin{subequations}\label{eq:Langmuir}
\begin{align}
    k_{\text{kin},i} \partial_t q_i = & k_{\text{eq},i}\left( \Lambda - \sum_{j \in \mathcal{C}_q}\left(\nu_j +\sigma_j\right) q_i \right)^{\nu_i} c_i - q_i c_\text{salt}^{\nu_i}\\
    &\partial_tq_{\text{salt}} = - \sum_{j \in \mathcal{C}_q}\nu_j \partial_tq_j
\end{align}
\end{subequations}

\section{Old results}
\begin{table}[tb]
\begin{center}
\caption{Results: Time to beat baseline. (P)~Passive, (A)~Active  refinement. (!) Not achieved.}\label{tb:results}

\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccc}
\hline
Method          & Best Obj.       & Reference   & Refined     \\
                & Value           & {[}min{]}   & {[}min{]}   \\ \hline
ECA             & \textbf{0.8592} & 77          & 106         \\
NSGA-II (E)     & 1.8495          & !           & !           \\
NSGA-II (M)     & 0.9553          & 22.5        & !           \\ \hline
(A) ECA         & 0.8656          & 48          & \textbf{84} \\
(P) ECA         & 0.8605          & 42          & 118.5       \\
(P) NSGA-II (E) & 1.1311          & 30          & !           \\
(P) NSGA-II (M) & 0.8967          & \textbf{18} & !           \\ \hline
Multi-Start     & 21.4299         & --          & --          \\
Reference       & 1.7705          & --          & --          \\
Refined         & 0.8875          & --          & --          \\ \hline
\end{tabular}%
}
\end{center}
\end{table}

==> tex/old/ifacexampletext.tex <==



Next we see a few subsections.

\subsection{Review Stage}

For submission guidelines, follow instructions on paper submission
system as well as the event website.

Note that conferences impose strict page limits, so it will be better
for you to prepare your initial submission in the camera ready layout
so that you will have a good estimate for the paper
length. Additionally, the effort required for final submission will be
minimal.

\subsection{Equations}

Some words might be appropriate describing equation~(\ref{eq:sample}), if 
we had but time and space enough. 

\begin{equation} \label{eq:sample}
{{\partial F}\over {\partial t}} = D{{\partial^2 F}\over {\partial x^2}}.
\end{equation}

See \cite{Abl:56}, \cite{AbTaRu:54}, \cite{Keo:58} and \cite{Pow:85}.

\subsubsection{Example.} This equation goes far beyond the
celebrated theorem ascribed to the great Pythagoras by his followers.

\begin{thm}   % use the thm environment for theorems
The square of the length of the hypotenuse of a right triangle equals
the sum of the squares of the lengths of the other two sides.
\end{thm}

\begin{pf}    % and the pf environment for proofs
The square of the length of the hypotenuse of a right triangle equals the sum of the squares 
of the lengths of the other two sides.
\end{pf}

%% There are a number of predefined theorem-like environments in
%% ifacconf.cls:
%%
%% \begin{thm} ... \end{thm}            % Theorem
%% \begin{lem} ... \end{lem}            % Lemma
%% \begin{claim} ... \end{claim}        % Claim
%% \begin{conj} ... \end{conj}          % Conjecture
%% \begin{cor} ... \end{cor}            % Corollary
%% \begin{fact} ... \end{fact}          % Fact
%% \begin{hypo} ... \end{hypo}          % Hypothesis
%% \begin{prop} ... \end{prop}          % Proposition
%% \begin{crit} ... \end{crit}          % Criterion

Of course LaTeX manages equations through built-in macros. You may
wish to use the \texttt{amstex} package for enhanced math
capabilities.

\subsection{Figures}

To insert figures, use the \texttt{graphicx} package. Although other
graphics packages can also be used, \texttt{graphicx} is simpler to
use. See  Fig.~\ref{fig:bifurcation} for an example.

\begin{figure}
\begin{center}
\includegraphics[width=8.4cm]{bifurcation}    % The printed column width is 8.4 cm.
\caption{Bifurcation: Plot of local maxima of $x$ with damping $a$ decreasing} 
\label{fig:bifurcation}
\end{center}
\end{figure}

Figures must be centered, and have a caption at the bottom. 

\subsection{Tables}
Tables must be centered and have a caption above them, numbered with
Arabic numerals. See table~\ref{tb:margins} for an example.

\begin{table}[hb]
\begin{center}
\caption{Margin settings}\label{tb:margins}
\begin{tabular}{cccc}
Page & Top & Bottom & Left/Right \\\hline
First & 3.5 & 2.5 & 1.5 \\
Rest & 2.5 & 2.5 & 1.5 \\ \hline
\end{tabular}
\end{center}
\end{table}

\subsection{Final Stage}

Authors are expected to mind the margins diligently.  Papers need to
be stamped with event data and paginated for inclusion in the
proceedings. If your manuscript bleeds into margins, you will be
required to resubmit and delay the proceedings preparation in the
process.

\subsubsection{Page margins.} See table~\ref{tb:margins} for the
page margins specification. All dimensions are in \emph{centimeters}.


\subsection{PDF Creation}

All fonts must be embedded/subsetted in the PDF file. Use one of the
following tools to produce a good quality PDF file:

\subsubsection{PDFLaTeX} is a special version of LaTeX by Han The
Thanh which produces PDF output directly using Type-1 fonts instead of
the standard \texttt{dvi} file. It accepts figures in JPEG, PNG, and PDF
formats, but not PostScript. Encapsulated PostScript figures can be
converted to PDF with the \texttt{epstopdf} tool or with Adobe Acrobat
Distiller.

\subsubsection{Generating PDF from PostScript} is the classical way of
producing PDF files from LaTeX. The steps are:

\begin{enumerate}
  \item Produce a \texttt{dvi} file by running \texttt{latex} twice.
  \item Produce a PostScript (\texttt{ps}) file with \texttt{dvips}.
  \item Produce a PDF file with \texttt{ps2pdf} or Adobe Acrobat
  Distiller.
\end{enumerate}

\subsection{Copyright Form}

IFAC will put in place an electronic copyright transfer system in due
course. Please \emph{do not} send copyright forms by mail or fax. More
information on this will be made available on IFAC website.


\section{Units}

Use SI as primary units. Other units may be used as secondary units
(in parentheses). This applies to papers in data storage. For example,
write ``$15\,\mathrm{Gb}/\mathrm{cm}^2$ ($100\,\mathrm{Gb}/\mathrm{in}^2$)''. 
An exception is when
English units are used as identifiers in trade, such as ``3.5 in
disk drive''. Avoid combining SI and other units, such as current in
amperes and magnetic field in oersteds. This often leads to confusion
because equations do not balance dimensionally. If you must use mixed
units, clearly state the units for each quantity in an equation.  The
SI unit for magnetic field strength $\mathbf{H}$ is $\mathrm{A}/\mathrm{m}$. However, if you wish to
use units of $\mathrm{T}$, either refer to magnetic flux density $\mathbf{B}$ or
magnetic field strength symbolized as $\mu_0\,\mathbf{H}$. Use the center dot to
separate compound units, e.g., ``$\mathrm{A} \cdot \mathrm{m}^2$''.

\section{Helpful Hints}

\subsection{Figures and Tables}

Figure axis labels are often a source of confusion. Use words rather
than symbols. As an example, write the quantity ``Magnetization'', or
``Magnetization M'', not just ``M''. Put units in parentheses. Do not
label axes only with units.  For example, write ``Magnetization
($\mathrm{A}/\mathrm{m}$)'' or ``Magnetization ($\mathrm{A} \mathrm{m}^{-1}$)'', not just
 ``$\mathrm{A}/\mathrm{m}$''. Do not
label axes with a ratio of quantities and units. For example, write
``Temperature ($\mathrm{K}$)'', not ``$\mbox{Temperature}/\mathrm{K}$''.

Multipliers can be especially confusing. Write ``Magnetization
($\mathrm{kA}/\mathrm{m}$)'' or ``Magnetization ($10^3 \mathrm{A}/\mathrm{m}$)''. Do not write
``Magnetization $(\mathrm{A}/\mathrm{m}) \times 1000$'' because the reader would not know
whether the axis label means $16000\,\mathrm{A}/\mathrm{m}$ or $0.016\,\mathrm{A}/\mathrm{m}$.

\subsection{References}

Use Harvard style references (see at the end of this document). With
\LaTeX, you can process an external bibliography database 
using \texttt{bibtex},\footnote{In this case you will also need the \texttt{ifacconf.bst}
file, which is part of the \texttt{ifaconf} package.}
or insert it directly into the reference section. Footnotes should be avoided as
far as possible.  Please note that the references at the end of this
document are in the preferred referencing style. Papers that have not
been published should be cited as ``unpublished''.  Capitalize only the
first word in a paper title, except for proper nouns and element
symbols.

\subsection{Abbreviations and Acronyms}

Define abbreviations and acronyms the first time they are used in the
text, even after they have already been defined in the
abstract. Abbreviations such as IFAC, SI, ac, and dc do not have to be
defined. Abbreviations that incorporate periods should not have
spaces: write ``C.N.R.S.'', not ``C. N. R. S.'' Do not use abbreviations
in the title unless they are unavoidable (for example, ``IFAC'' in the
title of this article).

\subsection{Equations}

Number equations consecutively with equation numbers in parentheses
flush with the right margin, as in (\ref{eq:sample}).  To make your equations more
compact, you may use the solidus ($/$), the $\exp$ function, or
appropriate exponents. Use parentheses to avoid ambiguities in
denominators. Punctuate equations when they are part of a sentence, as
in

\begin{equation} \label{eq:sample2}
\begin{array}{ll}
\int_0^{r_2} & F (r, \varphi ) dr d\varphi = [\sigma r_2 / (2 \mu_0 )] \\
& \cdot \int_0^{\inf} exp(-\lambda |z_j - z_i |) \lambda^{-1} J_1 (\lambda  r_2 ) J_0 (\lambda r_i ) d\lambda 
\end{array}
\end{equation}

Be sure that the symbols in your equation have been defined before the
equation appears or immediately following. Italicize symbols ($T$
might refer to temperature, but T is the unit tesla). Refer to
``(\ref{eq:sample})'', not ``Eq. (\ref{eq:sample})'' or ``equation
(\ref{eq:sample})'', except at the beginning of a sentence: ``Equation
(\ref{eq:sample}) is \ldots''.

\subsection{Other Recommendations}

Use one space after periods and colons. Hyphenate complex modifiers:
``zero-field-cooled magnetization''. Avoid dangling participles, such
as, ``Using (1), the potential was calculated'' (it is not clear who or
what used (1)). Write instead: ``The potential was calculated by using
(1)'', or ``Using (1), we calculated the potential''.

A parenthetical statement at the end of a sentence is punctuated
outside of the closing parenthesis (like this). (A parenthetical
sentence is punctuated within the parentheses.) Avoid contractions;
for example, write ``do not'' instead of ``don' t''. The serial comma
is preferred: ``A, B, and C'' instead of ``A, B and C''.


\section{Conclusion}

A conclusion section is not required. Although a conclusion may review
the main points of the paper, do not replicate the abstract as the
conclusion. A conclusion might elaborate on the importance of the work
or suggest applications and extensions.

